Efficient implementation of partitioned stiff exponential Runge-Kutta methods

Multiphysics systems are driven by multiple processes acting simultaneously, and their simulation leads to partitioned systems of differential equations. This paper studies the solution of partitioned systems of differential equations using exponential Runge-Kutta methods. We propose specific multiphysics implementations of exponential Runge-Kutta methods satisfying stiff order conditions that were developed in [Hochbruck et al., SISC, 1998] and [Luan and Osterman, JCAM, 2014]. We reformulate stiffly--accurate exponential Runge--Kutta methods in a way that naturally allows of the structure of multiphysics systems, and discuss their application to both component and additively partitioned systems. The resulting partitioned exponential methods only compute matrix functions of the Jacobians of individual components, rather than the Jacobian of the full, coupled system. We derive modified formulations of particular methods of order two, three and four, and apply them to solve a partitioned reaction-diffusion problem. The proposed methods retain full order for several partitionings of the discretized problem, including by components and by physical processes.

==> pexprk.tex <==
% !TEX root = Stiff-exp-partitioned.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Exponential Runge-Kutta methods written in partitioned form}
\label{sec:partitioned_exprk_methods}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

Consider the application of the \textit{transformed} exponential Runge--Kutta method \eqref{eqn:exp-RK-simple} to the component partitioned system \eqref{eqn:split-system-notation}:
% 
\begin{equation*}
\label{eqn:exp-RK-simple-component}
\begin{split}
U_i &\coloneqq V_i + W_i, \\
\begin{bmatrix} V_i \\  W_i \end{bmatrix} &= \begin{bmatrix} v_{n} \\  w_{n} \end{bmatrix} 
 +  h \, \begin{bmatrix}  \boldsymbol{\alpha}_{i,1}(h\Lone)\, \fone(u_n) \\  \boldsymbol{\alpha}_{i,1}(h\Ltwo)\, \ftwo(u_n)  \end{bmatrix} 
 + h\,\sum_{j=2}^{i-1} \begin{bmatrix}  \boldsymbol{\alpha}_{i,j}(h \Lone)\,\bigg(\fone(U_{j}) - \fone(u_n) \bigg) \\
 \boldsymbol{\alpha}_{i,j}(h \Ltwo)\,\bigg( \ftwo(U_{j}) - \ftwo(u_n) \bigg)  \end{bmatrix}, \quad i = 1, \hdots, s, \\
\begin{bmatrix} v_{n+1} \\  w_{n+1} \end{bmatrix}  &= \begin{bmatrix} v_{n} \\  w_{n} \end{bmatrix}  
+  h \, \begin{bmatrix}  \boldsymbol{\beta}_{1}(h\Lone)\, \fone(u_n) \\  \boldsymbol{\beta}_{1}(h\Ltwo)\, \ftwo(u_n)  \end{bmatrix} 
 + h\,\sum_{j=2}^{s} \begin{bmatrix}  \boldsymbol{\beta}_{j}(h \Lone)\,\bigg(\fone(U_{j}) - \fone(u_n) \bigg) \\
 \boldsymbol{\beta}_{j}(h \Ltwo)\,\bigg( \ftwo(U_{j}) - \ftwo(u_n) \bigg)  \end{bmatrix}.
\end{split}
\end{equation*} 
% 
Here $V_i$ and $W_i$ are the internal stages of the corresponding component ODEs, $U_i$ are the internal stages of the method obtained by adding the internal stages and the final one step solutions of the methods applied to the component ODEs, $v_n$ and $w_n$ are the current solutions of the component ODEs, $u_n$ is the current solution of the original ODE, $v_{n+1}$ and $w_{n+1}$ are the final one step solutions of the methods applied to the component ODEs.

By adding the internal stages and the final one step solutions of the methods applied to the component ODEs in a consistent manner, the above expressions lead to the partitioned Exponential Runge--Kutta formulation:
%
\begin{equation}
\label{eqn:exp-RK-simple-additive}
\begin{split}
U_i &= u_n +  h \, \boldsymbol{\alpha}_{i,1}(h\Lone)\, \fone(u_n) +  h \, \boldsymbol{\alpha}_{i,1}(h\Ltwo)\, \ftwo(u_n)  \\
& + h\,\sum_{j=2}^{i-1} \boldsymbol{\alpha}_{i,j}(h \Lone)\,\bigg(\fone(U_{j}) - \fone(u_n) \bigg)
+ h\,\sum_{j=2}^{i-1} \boldsymbol{\alpha}_{i,j}(h \Ltwo)\,\bigg( \ftwo(U_{j}) - \ftwo(u_n) \bigg), \quad i = 1, \hdots, s, \\
u_{n+1} &= u_{n} 
+  h \, \boldsymbol{\beta}_{1}(h\Lone)\, \fone(u_n) +  h \,  \boldsymbol{\beta}_{1}(h\Ltwo)\, \ftwo(u_n) \\
& + h\,\sum_{j=2}^{s}  \boldsymbol{\beta}_{j}(h \Lone)\,\bigg(\fone(U_{j}) - \fone(u_n) \bigg) 
+ h\,\sum_{j=2}^{s}  \boldsymbol{\beta}_{j}(h \Ltwo)\,\bigg( \ftwo(U_{j}) - \ftwo(u_n) \bigg).
\end{split}
\end{equation} 
%
Observe that method \eqref{eqn:exp-RK-simple-additive} applies matrix functions of $\Lone$ only to $\fone$, and matrix functions of $\Ltwo$ only to $\ftwo$. In this regard, it is a partitioned method.

\begin{remark}[Writing the partitioned method in terms of residuals]
\label{rem:partitioned-residual-form}
%
We seek to rewrite \eqref{eqn:exp-RK-simple-additive} in terms of residuals. For this we first write \eqref{eqn:exp-RK-simple-additive} in matrix form: 
%
\begin{equation*}
\begin{split}
\begin{bmatrix} U_2 - u_n \\  \vdots \\ U_s - u_n  \end{bmatrix} &=  
h\,\boldsymbol{\alpha}_{2:s,1}(h\Lone)\, \fone(u_n)  + h\,\boldsymbol{\alpha}_{2:s,1}(h\Ltwo)\, \ftwo(u_n) \\
& \quad + h\,\boldsymbol{\alpha}_{2:s,2:s}(h \Lone)\,\begin{bmatrix} \fone(U_{2}) - \fone(u_n) \\ \vdots \\ \fone(U_{s}) - \fone(u_n) \end{bmatrix}
+ h\,\boldsymbol{\alpha}_{2:s,2:s}(h \Ltwo)\,\begin{bmatrix} \ftwo(U_{2}) - \ftwo(u_n) \\ \vdots \\ \ftwo(U_{s}) - \ftwo(u_n) \end{bmatrix}.
\end{split}
\end{equation*} 
%
Next, we subtract back the linear terms from both sides:
%
\begin{equation*}
\begin{split}
& \left( \mathbf{I}_{s-1} - h\Lone\,\boldsymbol{\alpha}_{2:s,2:s}(h \Lone)  - h\Ltwo\,\boldsymbol{\alpha}_{2:s,2:s}(h \Ltwo) \right) \cdot \begin{bmatrix} U_2 - u_n \\  \vdots \\ U_s - u_n  \end{bmatrix} \\
& =  
h\,\boldsymbol{\alpha}_{2:s,1}(h\Lone)\, \fone(u_n)  + h\,\boldsymbol{\alpha}_{2:s,1}(h\Ltwo)\, \ftwo(u_n) \\
& \quad + h\,\boldsymbol{\alpha}_{2:s,2:s}(h \Lone)\,\begin{bmatrix} \gone(U_{2}) - \gone(u_n) \\ \vdots \\ \gone(U_{s}) - \gone(u_n) \end{bmatrix} + h\,\boldsymbol{\alpha}_{2:s,2:s}(h \Ltwo)\,\begin{bmatrix} \gtwo(U_{2}) - \gtwo(u_n) \\ \vdots \\ \gtwo(U_{s}) - \gtwo(u_n) \end{bmatrix}.
\end{split}
\end{equation*} 
%
Since $\boldsymbol{\alpha}_{2:s,2:s}$ are strictly lower triangular matrices, a formal inversion of the left hand side matrix is possible:
%
\[
\overline{\mathbf{E}}(h\Lone,h\Ltwo) \coloneqq \left( \mathbf{I}_{s-1} - h\Lone\,\boldsymbol{\alpha}_{2:s,2:s}(h \Lone)  - h\Ltwo\,\boldsymbol{\alpha}_{2:s,2:s}(h \Ltwo) \right)^{-1}.
\]
%
Using this inverse gives a partitioned method of exponential Runge--Kutta type \eqref{eqn:exp-RK}, whose coefficients $\overline{\mathbf{E}}(h\Lone,h\Ltwo)\boldsymbol{\alpha}(h \Lone)$ and $\overline{\mathbf{E}}(h\Lone,h\Ltwo)\boldsymbol{\alpha}(h \Ltwo)$ depend on both $\Lone$ and $\Ltwo$.
%
\end{remark}

\begin{remark}[Using two different methods]
A fully partitioned version of \eqref{eqn:exp-RK-simple} uses different schemes for different component ODEs:
% 
\begin{equation}
\label{eqn:exp-RK-simple-component-fullypartitioned}
\begin{split}
U_i &\coloneqq V_i + W_i, \\
\begin{bmatrix} V_i \\  W_i \end{bmatrix} &= \begin{bmatrix} v_{n} \\  w_{n} \end{bmatrix} 
 +  h \, \begin{bmatrix}  \boldsymbol{\alpha}^\one_{i,1}(h\Lone)\, \fone(u_n) \\  \boldsymbol{\alpha}^\two_{i,1}(h\Ltwo)\, \ftwo(u_n)  \end{bmatrix} 
 + h\,\sum_{j=2}^{i-1} \begin{bmatrix}  \boldsymbol{\alpha}^\one_{i,j}(h \Lone)\,\bigg(\fone(U_{j}) - \fone(u_n) \bigg) \\
 \boldsymbol{\alpha}^\two_{i,j}(h \Ltwo)\,\bigg( \ftwo(U_{j}) - \ftwo(u_n) \bigg)  \end{bmatrix}, \quad i = 1, \hdots, s,\\
\begin{bmatrix} v_{n+1} \\  w_{n+1} \end{bmatrix}  &= \begin{bmatrix} v_{n} \\  w_{n} \end{bmatrix}  
+  h \, \begin{bmatrix}  \boldsymbol{\beta}^\one_{1}(h\Lone)\, \fone(u_n) \\  \boldsymbol{\beta}^\two_{1}(h\Ltwo)\, \ftwo(u_n)  \end{bmatrix} 
 + h\,\sum_{j=2}^{s} \begin{bmatrix}  \boldsymbol{\beta}^\one_{j}(h \Lone)\,\bigg(\fone(U_{j}) - \fone(u_n) \bigg) \\
 \boldsymbol{\beta}^\two_{j}(h \Ltwo)\,\bigg( \ftwo(U_{j}) - \ftwo(u_n) \bigg)  \end{bmatrix}.
\end{split}
\end{equation} 
%
Notice the supercase index on $\boldsymbol{\alpha}$ and $\boldsymbol{\beta}$ coefficients.
\end{remark}
%

==> pexprk_convergence_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence of PEXPRK methods}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

We consider the additive partitioned system in component form \eqref{eqn:component-form-additive-ode} and  perform  a linear-nonlinear splitting of the form \eqref{eqn:component-split-ode-semilinear}:
%
%
\begin{equation}
\label{eqn:additive-split-ode-semilinear}
\begin{split}
y' &= \begin{bmatrix} v' \\ w' \end{bmatrix} =
\begin{bmatrix} \fone(v + w) \\ \ftwo(v + w) \end{bmatrix} =
\begin{bmatrix}  \Lone \cdot v  + \gone(v , w) \\ \Ltwo \cdot w + \gtwo(v , w) \end{bmatrix} 
= \Lb \cdot y  + \g(y),
\end{split}
\end{equation}
%
where $\Lone$ and $\Ltwo$ are linear operators that contain the stiffnesses of $\fone$ and $\ftwo$, respectively, $\gone$ and $\gtwo$ are the corresponding non-linear remainder functions. 
We have
%
\begin{equation}
\label{eqn:nonlinear-remainder}
\Lb \coloneqq \begin{bmatrix} \Lone & \Zero \\  \Zero & \Ltwo \end{bmatrix}, \quad
\g(y) \coloneqq \begin{bmatrix} \gone(v, w) \\ \gtwo(v, w) \end{bmatrix} 
\coloneqq \begin{bmatrix} \fone(v+ w) - \Lone \cdot v \\ \ftwo(v+ w) - \Ltwo \cdot w \end{bmatrix}.
\end{equation}
%
For simplicity we consider the case where exact Jacobians are used in the partition, $\Lone = \Jone(y_n)$ and $\Ltwo = \Jtwo(y_n)$. The Jacobian of the non-linear remainder, $\g$, has the structure:
%
\begin{equation}
\g'(y_n)= \f'(y_n)-\Lb =
\begin{bmatrix} \mathbf{0} & \Lone \\ \Ltwo & \mathbf{0} \end{bmatrix}.
\end{equation}
%
\textcolor{blue}{Note that the standard linear-nonlinear splitting \eqref{eqn:lin-nonlin-split-ode} using the full Jacobian evaluated at $y_n$ as the linear operator \eqref{eqn:component-form-additive-ode} leads to 
%
\begin{equation}
\label{eqn:additive-split-ode-standard-semilinear}
\begin{split}
y' &= \begin{bmatrix} v' \\ w' \end{bmatrix} =
\begin{bmatrix} \fone(v + w) \\ \ftwo(v + w) \end{bmatrix} =
\begin{bmatrix}  \Lone \cdot (v + w)  + \g^{\textnormal{standard}, \{1\}}(v , w) \\ \Ltwo \cdot (v + w) + \g^{\textnormal{standard}, \{2\}}(v , w) \end{bmatrix} 
= \J(y_n) \cdot y  + \g^{\textnormal{standard}}(y),
\end{split}
\end{equation}
%
where the nonlinear remainder is
%
\begin{equation}
\label{eqn:standard-remainder}
\g^{\textnormal{standard}}(y) = \begin{bmatrix} \fone(v+ w) - \Lone \cdot (v + w) \\ \ftwo(v+ w) - \Ltwo \cdot (v+w) \end{bmatrix}.
\end{equation}
%
We now follow closely the analysis \cite{luan2014,luan2014a,luan2014b,hochbruck2009} applied to the component split formulation \eqref{eqn:additive-split-ode-semilinear}. We make the following additional assumption:
%
\begin{assumption}
\label{ass:two-for-additive-splitting}
The system \eqref{eqn:additive-split-ode-standard-semilinear} obeys Assumptions \ref{ass:one} and \ref{ass:two}. In particular, there is an initial condition $v_0,w_0$ with $y_0 = [v_0; w_0]$ such that each component equation \eqref{eqn:additive-split-ode-standard-semilinear} admits a sufficiently smooth solution $v,w : [0,T] \to X$ with derivatives in $X$. 
\end{assumption}}

Higher derivatives of our remainder \eqref{eqn:nonlinear-remainder} and of the standard remainder \eqref{eqn:standard-remainder}  coincide
%
\[
\g^{(k)}(y) = \left( \g^{\textnormal{standard}} \right)^{(k)} (y), \quad k \ge 2,
\]
%
and are therefore uniformly bounded if Assumption \ref{ass:two-for-additive-splitting} holds. The first derivatives, however, require a closer look. The Jacobian of the standard remainder \eqref{eqn:standard-remainder} is
%
\begin{equation}
\label{eqn:jacobian-standard-remainder}
\bigl( \g^{\textnormal{standard}}\bigr)'(y) = 
\begin{bmatrix} {\J}^\one(y) - \Lone & {\J}^\one(y)-\Lone \\ {\J}^\two(y) - \Ltwo & {\J}^\two(y) - \Ltwo \end{bmatrix},
\end{equation}
%
and is uniformly bounded by Assumption \ref{ass:two-for-additive-splitting}.
%
The Jacobian of our nonlinear reminder \eqref{eqn:nonlinear-remainder}
%
\begin{equation}
\g'(y) = 
\begin{bmatrix} {\J}^\one(y)-\Lone & {\J}^\one(y) \\ {\J}^\two(y) & {\J}^\two(y) - \Ltwo \end{bmatrix}
\end{equation}
%
is not, due to the presence of the stiff Jacobians (and not Jacobian differences) in off-diagonal positions. However, we have the following.

\begin{remark}
The product of a function $h \varphi_k(h\Lb)$ with $k \ge 1$ and the Jacobian is uniformly bounded. This product reads:
%
\begin{equation}
\label{eqn:phi-jac}
\begin{split}
h \varphi_k(h\Lb)\,\g'(u) &= 
\begin{bmatrix} h \varphi_k(h \Lone) & \Zero \\  \Zero & h \varphi_k(h \Ltwo) \end{bmatrix} \cdot
\begin{bmatrix} {\J}^\one-\Lone & {\J}^\one \\ {\J}^\two & {\J}^\two - \Ltwo \end{bmatrix} \\
&= 
\begin{bmatrix} h \varphi_k(h \Lone)\, \left( {\J}^\one-\Lone \right) & h \varphi_k(h \Lone)\,{\J}^\one \\ h \varphi_k(h \Ltwo)\,{\J}^\two & h \varphi_k(h \Ltwo)\, \left( {\J}^\two - \Ltwo \right) \end{bmatrix}.
\end{split}
\end{equation}
%
The diagonal blocks are uniformly bounded by Assumption \ref{ass:two-for-additive-splitting}. The off-diagonal blocks are also uniformly bounded, since each term on the right of
%
\begin{equation}
\label{eqn:phi-jac-bound}
\begin{split}
h \varphi_k(h \Lone)\,{\J}^\one &= h \varphi_k(h \Lone)\, \left( {\J}^\one-\Lone \right) + \varphi_k(h \Lone)\,h \Lone \\
&= h \varphi_k(h \Lone)\, \left( {\J}^\one-\Lone \right) +  \left(\varphi_{k-1}(h \Lone) - \frac{\Id}{(k - 1)!}\right),
\end{split}
\end{equation}
% 
is uniformly bounded.
\end{remark}

It was shown in  \cite{luan2014,luan2014a,luan2014b,hochbruck2009} that the local error of the method has the form:
%
\begin{equation}
\label{eqn:local-error}
\begin{split}
e_n &= h^2\, \Psi_2(h\Lb)\, g'(\widetilde{y})\, \widetilde{y}' 
+ h^3\, \Psi_2(h\Lb)\,\left(   g'(\widetilde{y})\,\widetilde{y}'' + g^{(2)}(\widetilde{y})(\widetilde{y}',\widetilde{y}') \right) \\
&\quad + h^3 \sum_{j=2}^s b_j(h\Lb)\, g'(\widetilde{y})\, \psi_{2,j}(h\Lb)\, g'(\widetilde{y})\, \widetilde{y}'  + \dots \\
&= h\, \Psi_2(h\Lb)\, h g'(\widetilde{y})\, \widetilde{y}' 
+ h^2\, \Psi_2(h\Lb)\,\left(  h g'(\widetilde{y})\,\widetilde{y}'' + h g^{(2)}(\widetilde{y})(\widetilde{y}',\widetilde{y}') \right) \\
&\quad + h \sum_{j=2}^s b_j(h\Lb)\, h g'(\widetilde{y})\, \psi_{2,j}(h\Lb)\, h g'(\widetilde{y})\, \widetilde{y}'  + \dots 
\end{split}
\end{equation}
%
It was shown in  \cite[Section 3.3]{luan2014b} that the local error of the method has the form:
%
\begin{equation}
\label{eqn:local-error}
\begin{split}
e_n &= h^2\, \Psi_2(h\Lb)\, g'(\widetilde{y})\, \widetilde{y}' 
+ h^3\, \Psi_3(h\Lb)\,\left(   g'(\widetilde{y})\,\widetilde{y}'' + g^{(2)}(\widetilde{y})(\widetilde{y}',\widetilde{y}') \right) \\
&\quad + h^3 \sum_{j=2}^s b_j(h\Lb)\, g'(\widetilde{y})\, \psi_{2,j}(h\Lb)\, g'(\widetilde{y})\, \widetilde{y}'  + \dots \\
&= h\, \Psi_2(h\Lb)\, h g'(\widetilde{y})\, \widetilde{y}' 
+ h^2\, \Psi_3(h\Lb)\,\left(  h g'(\widetilde{y})\,\widetilde{y}'' + h g^{(2)}(\widetilde{y})(\widetilde{y}',\widetilde{y}') \right) \\
&\quad + h \sum_{j=2}^s b_j(h\Lb)\, h g'(\widetilde{y})\, \psi_{2,j}(h\Lb)\, h g'(\widetilde{y})\, \widetilde{y}'  + \dots 
\end{split}
\end{equation}with
%
\[
\Psi_j(z) = \sum_{i=2}^s b_i(z) \, \frac{c_i^{j-1}}{(j-1)!} - \varphi_j(z).
\]
%
and $\psi_{i,j}$ defined in \eqref{eqn:psi-ij}.

The coefficients of the powers of $h$ in \eqref{eqn:local-error} contain higher derivatives of the remainder, which are uniformly bounded, and the Jacobian of the remainder multiplied from the left by either $h\,\Psi_j(h\Lb)$, $j\ge 2$, or $h\,\psi_{i,j}(h\Lb)$, or $h\, b_i(h\Lb)$, or $h\, a_{i,j}(h\Lb)$.
%
Consequently, the coefficients of the powers of $h$ in the error expansion \eqref{eqn:local-error} are uniformly bounded if each of these products are uniformly bounded. 


%
\begin{assumption}
\label{ass:method-coefficients}
The coefficients of the exponential Runge-Kutta method are defined such that all functions $z\,b_i(z)$ and $z\, a_{i,j}(z)$, $i,j=2, \dots, s$  are analytical.  In particular, the assumption holds if  the coefficients $b_i(z)$ and $a_{i,j}(z)$ are linear combinations of functions $\varphi_k(z)$ and their scaled variants, with $k \ge 1$.
\end{assumption}

Using a similar reasoning as in \eqref{eqn:phi-jac}, \eqref{eqn:phi-jac-bound}, the following  result is established.
%
\begin{lemma}
If Assumption \ref{ass:method-coefficients} holds then the coefficients of the local error expansion \eqref{eqn:local-error} are uniformly bounded independent of the stiffness of the component systems. \textcolor{red}{However, this error expansion is only $\mathcal{O}(h)$.}
\end{lemma}

Next, we are concerned with the stability of the method. 
%
From \eqref{eqn:nonlinear-remainder}--\eqref{eqn:standard-remainder} we have:
%
\[
\begin{split}
%\g(y)& = \g^{\textnormal{standard}}(y) +  \begin{bmatrix} \Lone \cdot w \\  \Ltwo \cdot v \end{bmatrix}, \\
\g(y_1) - \g(y_2) &= \g^{\textnormal{standard}}(y_1) - \g^{\textnormal{standard}}(y_2)  +  \begin{bmatrix} \Lone \cdot (w_1-w_2) \\  \Ltwo \cdot (v_1 - v_2) \end{bmatrix}.
\end{split}
\]
%
Clearly $\g$ does not have a moderate Lipschitz constant due to the presence of the stiff linear terms. However, we make the following remark.

\begin{remark}
The function $h \varphi_k(h\Lb)\, g(y)$, $k\ge 1$, is Lipschitz continuous with a moderate Lipschitz constant. We have that:
%
\[
\begin{split}
h \varphi_k(h\Lb) \g(y_1) - h \varphi_k(h\Lb)\g(y_2)  &= h \varphi_k(h\Lb) \left( \g^{\textnormal{standard}}(y_1) - \g^{\textnormal{standard}}(y_2) \right)  +  h \varphi_k(h\Lb) \, \Lb\, \begin{bmatrix} w_1-w_2 \\  v_1 - v_2 \end{bmatrix}, \\
\Vert h \varphi_k(h\Lb) \g(y_1) - h \varphi_k(h\Lb)\g(y_2) \Vert &\le h \,\Vert \varphi_k(h\Lb) \Vert\cdot L_\g^{\textnormal{standard}}\cdot \Vert y_1 - y_2 \Vert
+ \Vert h \varphi_k(h\Lb) \, \Lb \Vert \cdot \Vert y_1 - y_2 \Vert.
\end{split}
\]
%
Here $L_\g^{\textnormal{standard}}$ is the moderate Lipschitz constant of the standard remainder. Both $h \varphi_k(h\Lb)$ and $h \varphi_k(h\Lb) \, \Lb$ operators are uniformly bounded for $k\ge 1$ under the assumptions we made.
\end{remark}

Regarding stability of the method, it was shown in  \cite{luan2014,luan2014a,luan2014b} that the difference of two numerical solutions started at two different approximations of the solution at $t_k$, (i.e.) $y_k$ and $z_k$, after $n - k$ steps has the form:
%
\[
y_n - z_n = e^{(\sum_{m=k}^{n-1} h_m)\, \Lb} \, (y_k - z_k) + \sum_{m=k}^{n-1}  e^{(\sum_{\ell=m+1}^{n-1} h_\ell)\, \Lb} \, 
\sum_{i=1}^s \left(h_m b_i(h_m\Lb)\right) \, \left( g(Y_{m,i}) - g(Z_{m,i}) \right).
\]
%
If the functions $h b_i(h\Lb)\, g(y)$ are Lipschitz continuous then stability follows along the lines of the proof in \cite{luan2014,luan2014a,luan2014b}. We have the following.

\begin{lemma}
If Assumption \ref{ass:method-coefficients} holds then the functions $h b_i(h\Lb)\, g(y)$ are Lipschitz continuous, and therefore the partitioned exponential Runge-Kutta scheme is stable.
\end{lemma}

The stability and accuracy properties imply convergence. 
%
\begin{lemma}
If Assumptions \ref{ass:two-for-additive-splitting} and \ref{ass:method-coefficients} hold, then the PEXPRK method converges with the order given by the order conditions.
\end{lemma}

